DISCO: accurate Discrete Scale Convolutions

Scale is often seen as a given, disturbing factor in many vision tasks. When doing so it is one of the factors why we need more data during learning. In recent work scale equivariance was added to convolutional neural networks. It was shown to be effective for a range of tasks. We aim for accurate scale-equivariant convolutional neural networks (SE-CNNs) applicable for problems where high granularity of scale and small kernel sizes are required. Current SE-CNNs rely on weight sharing and kernel rescaling, the latter of which is accurate for integer scales only. To reach accurate scale equivariance, we derive general constraints under which scale-convolution remains equivariant to discrete rescaling. We find the exact solution for all cases where it exists, and compute the approximation for the rest. The discrete scale-convolution pays off, as demonstrated in a new state-of-the-art classification on MNIST-scale and on STL-10 in the supervised learning setting. With the same SE scheme, we also improve the computational effort of a scale-equivariant Siamese tracker on OTB-13.

==> sections/geom_figure.tex <==
\begin{figure*}[th]
  \centering
    \includegraphics[width=0.9\linewidth]{pics/geom_supp.png}
  \caption{Images and their scale fields produced by the DISCO model trained to contrast the scales. \textbf{Left}: M. C. Escher drawing. Produced scale field captures that the scale of the pattern diminishes from center to borders. \textbf{Center}: the scale of the cars diminishes as they drive away from the camera. DISCO scale field reveals that cars in the bottom-left corner are of a bigger scale than in the top-right. \textbf{Right}: DISCO scale field captures that products on the shelf decrease in scale from closer shelves on the sides to the center.}
  \label{fig:scene_geom_supp}
\end{figure*}
